Foundation Models for Video Understanding: A Survey

Video Foundation Models (ViFMs) aim to learn a general-purpose representation for various video understanding tasks. Leveraging large-scale datasets and powerful models, ViFMs achieve this by capturing robust and generic features from video data. This survey analyzes over 200 video foundational models, offering a comprehensive overview of benchmarks and evaluation metrics across 14 distinct video tasks categorized into 3 main categories. Additionally, we offer an in-depth performance analysis of these models for the 6 most common video tasks. We categorize ViFMs into three categories: 1) Image-based ViFMs, which adapt existing image models for video tasks, 2) Video-Based ViFMs, which utilize video-specific encoding methods, and 3) Universal Foundational Models (UFMs), which combine multiple modalities (image, video, audio, and text etc.) within a single framework. By comparing the performance of various ViFMs on different tasks, this survey offers valuable insights into their strengths and weaknesses, guiding future advancements in video understanding. Our analysis surprisingly reveals that image-based foundation models consistently outperform video-based models on most video understanding tasks. Additionally, UFMs, which leverage diverse modalities, demonstrate superior performance on video tasks. We share the comprehensive list of ViFMs studied in this work at: \url{https://github.com/NeeluMadan/ViFM_Survey.git}

==> figures/finetuned_results.tex <==
\pgfplotsset{compat=newest}
\definecolor{IFM}{HTML}{dad2ff}
\definecolor{VFM}{HTML}{ad9bff}
\definecolor{UFM}{HTML}{7355ff}
\definecolor{SPC}{RGB}{240,83,50}

\pgfplotstableread[col sep=comma]{
	Benchmarks, Image-Based, Video-Based, Universal-Model, Specialist
	
	2011,90.6,90.0,91.1,87.7
	2012,58.7,55.2,89.3,54.3
	2013,86.8,84.1,0,82.7
	2014,74.7,77.0,77.2,69.5
	}\mytableA

\pgfplotstableread[col sep=comma]{
	Year, Image-Based, Video-Based, Universal-Model, Specialist
	
	2011,58.5,48.8,63.9,54.0
	2012,70.4,59.8,72.0,55.0
	2013,43.0,27.1,34.4,27.7
	
	}\mytableB

\pgfplotstableread[col sep=comma]{
	Year, Image-Based, Video-Based, Universal-Model, Specialist
	
	2011,73.2,62.5,80.3,60.8
	2012,123.4, 150.7, 195.6,120.6
	2013,128.0,127.0,198.8,133
	
	}\mytableC

\begin{figure}
\begin{tabular}{cc}
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \begin{tikzpicture}
      % Your axis definition for the first plot (Action Recognition)
      \end{tikzpicture}
    \caption{Action Recognition}
  \end{subfigure} &
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \begin{tikzpicture}
      % Your axis definition for the second plot (Video Retrieval)
      \end{tikzpicture}
    \caption{Video Retrieval}
  \end{subfigure} \\
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \begin{tikzpicture}
      % Your axis definition for the third plot (Video Captioning)
      \end{tikzpicture}
    \caption{Video Captioning}
  \end{subfigure} 
  &  
  \caption{Comparison of Action Recognition, Video Retrieval, and Video Captioning}
\end{tabular}
\end{figure}


==> figures/method_analysis.tex <==

% \begin{figure*}[htbp]
%     \centering
%     \includegraphics[width=\textwidth]{figures/combined_new.pdf}
%     \caption{\textbf{A general analysis of VFMs across several video tasks}:  Video-specific models \textit{significantly} lag behind Image-specific models in 9/10 cases. This indicates the need for curating video-data and improving video-based modelling. Unified Models outperform task-specific specialists. IM: Image-Model, VM: Video-Model, UM: Unified Model, Specialist: Task-specific finetuned model.}
%     \label{fig:method_description}
% \end{figure*}

